Learning on-the-fly quasi-stationarity diagnostics from low-dimensional surrogates

Accelerated dynamics methods, such as parallel replica dynamics, require estimates of the decorrelation time, after which a process trapped in one of its metastable states is distributed according to the quasi-stationary distribution (QSD). In a method proposed by Binder, Leli\`evre and Simpson, decorrelation times are defined by coupling a particle approximation of the non-linear conditioned probability flow of the process with MCMC-inspired diagnostics. We explore an alternative to MCMC diagnostics, based on coarse-graining of non-linear probability flows and simulation-based inference. We first develop a coarse-graining framework for killed Markov jump processes conditioned on survival, proving uniform-in-time, non-asymptotic estimates approximating the non-linear probability flow of the true process by the non-linear flow of a surrogate process, defined with a collective variable. The framework does not assume reversibility of the true process, and also gives bounds which scale explicitly in an adiabatic regime. Motivated by these results, we then construct a quasi-stationarity diagnostic using simulation-based inference: a recurrent neural network (RNN), trained on particle approximations of non-linear effective flows, estimates posterior probabilities of decorrelation. The learned diagnostic is then transferred to collective-variable traces of high-dimensional particle approximations. We investigate the behavior and robustness of this diagnostic on a set of numerical experiments, comparing it to the MCMC diagnostic of Binder et al.\ on both synthetic examples and a molecular system, in and out of its training prior distribution. When its prior assumptions hold, the RNN diagnostic outperforms the MCMC diagnostic in ROC analysis, is less conservative, fails less often, and has an interpretable decision threshold.

==> tables/diagnostic_cost_table.tex <==
\begin{tabular}{rr r rr rr}
\toprule
 & & MD & \multicolumn{2}{c}{NN} & \multicolumn{2}{c}{Gelman--Rubin} \\
\cmidrule(lr){3-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
$N$ & $\tau$ & wall-clock (ms) & ($\mu$s) & / wall-clock & ($\mu$s) & / wall-clock \\
\midrule
25 & 100$\Delta t$ & 3.6 & 33 & 0.92\% & 0.4 & 0.012\% \\
\bottomrule
\end{tabular}


==> tables/robustness_table_exits.tex <==
\begin{tabular}{l l c cc cc}
\toprule
 & & & \multicolumn{2}{c}{exit side} & \multicolumn{2}{c}{asymmetry} \\
\cmidrule(lr){4-5}\cmidrule(lr){6-7}
$D_{\mathrm{d}}$ & diagnostic & $\Delta\bar\tau$ & $\max|\Delta p|$ & out & range & $0\notin$ CI \\
\midrule
\multirow{5}{*}{$0.05$} & reference & -- & -- & -- & +1.1\% & -- \\
 & RNN, $\alpha=0.1$ & -0.4\% & 0.006 & 0 & [-2.0\%, +5.0\%] & 1 \\
 & RNN, $\alpha=0.05$ & -1.4\% & 0.012 & 0 & [-0.3\%, +2.9\%] & 0 \\
 & GR, $\alpha=0.1$ & -1.3\% & 0.013 & 0 & [+0.0\%, +3.3\%] & 0 \\
 & GR, $\alpha=0.05$ & -1.5\% & 0.009 & 0 & [-1.3\%, +2.9\%] & 0 \\
\midrule
\multirow{5}{*}{$1$} & reference & -- & -- & -- & -0.2\% & -- \\
 & RNN, $\alpha=0.1$ & -1.1\% & 0.054 & 4 & [-12.4\%, +22.9\%] & 4 \\
 & RNN, $\alpha=0.05$ & -0.7\% & 0.039 & 3 & [-12.3\%, +13.6\%] & 5 \\
 & GR, $\alpha=0.1$ & -0.5\% & 0.022 & 0 & [-4.0\%, +6.0\%] & 2 \\
 & GR, $\alpha=0.05$ & -0.4\% & 0.010 & 0 & [-3.4\%, +2.1\%] & 0 \\
\bottomrule
\end{tabular}

